A census of young stellar population associated with the Herbig Be star HD 200775

The region surrounding the well-known reflection nebula, NGC 7023, illuminated by a Herbig Be star, HD 200775, located in the dark cloud L1174 is studied in this work. Based on the distances and proper motion values from Gaia DR2 of 20 previously known young stellar object candidates, we obtained a distance of 335$\pm$11 pc to the cloud complex L1172/1174. Using polarization measurements of the stars projected on the cloud complex, we show additional evidence for the cloud to be at $\sim$ 335 pc distance. Using this distance and proper motion values of the YSO candidates, we searched for additional comoving sources in the vicinity of HD 200775 and found 20 new sources which show low infrared excess emission and are of age $\sim$ 1 Myr. Among these, 10 YSO candidates and 4 newly identified comoving sources are found to show X-ray emission. Three of the four new sources for which we have obtained optical spectra show H$\alpha$ in emission. About 80% of the total sources are found within $\sim$ 1 pc distance from HD 200775. Spatial correlation of some of the YSO candidates with the Herschel dust column density peaks suggests that star formation is still active in the region and may have been triggered by HD 200775.

==> table_pm_ref.tex <==
\begin{table}
	\centering
	\caption{Details of the four 1$^{\circ}$ square reference fields selected around L1172/1174.}
	\label{tab:pm_ref}
	\begin{tabular}{p{1.2cm}p{1.5cm}p{1.5cm}p{2cm}}\hline
		Field  &RA (J2000)  &Dec (J2000)    & \# of stars$^{\dagger}$\\
		        &($^{\circ}$)&($^{\circ}$)  &\\\hline\hline
		%Field 1&315.403923	&$+$69.159951	&0\\
		%Field 2&315.403923	&$+$67.160139	&1\\
		%Field 3&312.713942	&$+$68.163271	&3\\
		%Field 4&318.086142	&$+$68.163271	&2\\
		tail-east & 318.79282 &$+$67.174828	&1\\
		tail & 316.21048 &$+$67.206136	&0\\
		tail-west &	313.56081 &$+$67.197843	&0\\
        \hline     
	\end{tabular}\\
	
	$^{\dagger}$Number of comoving stars found within the constraint of 5$\times$MAD about the median values of the distance, $\mu_{\star}$ and $\mu_{\delta}$ obtained for YSO candidates. 
\end{table}
